Relative stability toward diffeomorphisms indicates performance in deep nets

Understanding why deep nets can classify data in large dimensions remains a challenge. It has been proposed that they do so by becoming stable to diffeomorphisms, yet existing empirical measurements support that it is often not the case. We revisit this question by defining a maximum-entropy distribution on diffeomorphisms, that allows to study typical diffeomorphisms of a given norm. We confirm that stability toward diffeomorphisms does not strongly correlate to performance on benchmark data sets of images. By contrast, we find that the stability toward diffeomorphisms relative to that of generic transformations $R_f$ correlates remarkably with the test error $\epsilon_t$. It is of order unity at initialization but decreases by several decades during training for state-of-the-art architectures. For CIFAR10 and 15 known architectures, we find $\epsilon_t\approx 0.2\sqrt{R_f}$, suggesting that obtaining a small $R_f$ is important to achieve good performance. We study how $R_f$ depends on the size of the training set and compare it to a simple model of invariant learning.

==> checklist.tex <==
\section*{Checklist}
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} Our work seeks to discover empirical laws and, as such, raises more questions than it answers. We list some of them in the conclusion.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{} We don't foresee possible negative societal consequences of our work. On the contrary, we think our work can positively contribute to the effort that the machine learning Community is putting into developing interpretable AI. 
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}, we provide links to github repositories, code and instructions on how to run it are found there.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} we provide major details in the main text and specific details in Appendix E.1.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{} We specify that -- to the benefit of figures clarity -- error estimates are not always reported in the main text. In these cases, we provide error estimates in Appendix E.3.
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} We provide GPUs type and the wall time needed to run each individual training performed. We provide an estimate for the total number of compute time employed for this work.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} We use existing data-sets and architectures, all properly cited, to the best of our knowledge.
  \item Did you mention the license of the assets?
    \answerYes{} For the models we did not implement ourselves, the license is present in the \texttt{models} folder of our github repository.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{} We provide a new library for generating max-entropy diffeomorfisms on images together with the link to the corresponding github repository.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> old sections/DiffeomorphismStability.tex <==
% this section should only focus on the definition of D, and on the fact that we can extract from it an estimate of the typical gradient in the direction of diffeo. 
% The choice delta=1 results from the compromise small delta vs insensitivity to interpolation method. 

%If neural nets can beat the curse of dimensionality by learning invariances present in the data, and if smooth deformations of the images are one such invariance, the typical gradient of $f$ around the manifold of diffeomorphisms...

Our working hypothesis is that neural nets can beat the course of dimensionality by learning invariances present in the data and we identify smooth deformations of the images as one such invariance. In order to investigate our working hypothesis, on the line of what we presented in the previous section, we propose here a way of measuring the sensitivity of a network function when the input $x$ moves along the manifold of diffeomorphisms.

\paragraph{Definition} 
To study how the typical gradients of $f$ evolve, when exploring the manifold of diffeomorphisms around data-points, we define the roughness measure
%In order to quantify the neural networks stability towards diffeomorphisms, we define the roughness measure of $f$ along the manifold of diffeomorphisms:
\begin{equation}
    D_f(T, c) = \frac{\langle \|f(\tau x) - f(x)\|^2\rangle_{x, \tau}}{\langle \|f(x) - f(z)\|^2\rangle_{x, z}}
    \label{eq:D_f}
\end{equation}
where again $x, z \in \mathcal D_{te}$ and $\tau$ are diffeomorphisms generated at temperature $T$ and with high-frequency cut-off $c$. 
% \footnote{The equality $\|\tau x - x\| = \sqrt T$ holds for small displacement fields as $\tau x (s) = x(\tau^{-1}(s)) = x(s - \sqrt{T}\xi(s)) \approx x(s) - \sqrt{T}\xi(s) \nabla x(s)$.}
$D_f$ is a measure of the regularity of $f$ along the manifold of diffeomorphisms. 

\paragraph{Empirical Results}
We measure $D_f$ for a ResNet trained on a set of benchmark datasets -- Figure \ref{fig:D_f_resnet} (analogous plots for EfficientNet are shown in Appendix \ref{app:more_experiments}, Figure \ref{fig:D_f_effnet}). We report the results as a function of the typical pixel displacement $\delta$ and high-frequency cut-off $c$. We chose to report the dependence on $\delta$ instead of $T$ as the deformation magnitude $\|\tau x - x\|$ naturally depends on it -- cf. Appendix \ref{app:typical_pix_dis_deform_magn}. Moreover its magnitude is easier to interpret, being it the typical pixel displacement. We recall that $\delta \sim \sqrt T$. 

The first observation we make is that all the nets get less sensitive to diffeomorphisms with training (dashed = init, full lines = trained), the lesser for smaller cut-off values (light colors). Moreover, we notice that at small displacements ($\delta\to 0$), the choice of interpolation method matters (blue and red curves drift apart). For this reason, in the next Section we focus our study of diffeomorphisms compression at $\delta=1$.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/diffeo_resnet.pdf}
    \caption{\textbf{Sensitivity on the manifold of diffeomorphisms, $D_f$.} Typical roughness of $f_0$ (init) and $f$ (trained) along the manifold of diffeomorphisms around data-points as a function of the typical pixel displacement $\delta$ ($x-$axis), for different cut-off values $c$ (lighter colors correspond to smaller $c$). Each panel corresponds to a ResNet trained on a different data-set. The "trained" curves are always below the "init" ones, indicating an increased invariance after training. The curves colors indicate the interpolation method; methods start matching from $\delta \sim 1$.
    \textit{Statistics:} MNIST, FMNIST and CIFAR10 results are log-averaged over 20 different nets realizations and trainings. For ImageNet, one instance of a pre-trained net has been downloaded from \texttt{torch.hub}. The averages in $x$ are taken over 100 data samples and noise realizations.}
    \label{fig:D_f_resnet}
\end{figure}

==> old sections/NTK.tex <==
% \paragraph{Learning with kernels}  A kernel $K$ is a function that acts on two data-points $x$ and $z$ and outputs a similarity measure between the them. As an example, a Laplace Kernel can be defined as
% \begin{equation}
%     K(x, z) = e^{-\|x - z\|}.
% \end{equation}
% In machine learning, kernel methods are a class of algorithms that use such functions to learn from data.

In this section, we study the properties of the \textit{neural tangent kernel} (NTK) \cite{jacot2018neural}. In particular, we examine whether also the NTK shows the invariance toward diffeomorphisms we measured for the network function.

\paragraph{NTK} Consider the gradient descent dynamics 
$\dot W = -\nabla_W \mathcal{L}$, where $\mathcal{L} = \sum_\mu l(f(x^\mu; W), y^\mu)$ is the train loss for a given choice of loss function $l$.
In function space, the dynamics reads
\begin{align}
    \dot f(x) &= \nabla_W f(x)\cdot \dot W \\
    & = -\sum_\mu \nabla_W f(x)\cdot \nabla_W f(x^\mu)\, l'(f(x^\mu; W), y^\mu)
\end{align}
and only depends on a kernel $\Theta(x, z) = \nabla_W f(x)\cdot \nabla_W f(z)$
coined the \textit{neural tangent kernel} \cite{jacot2018neural}. In general, the NTK evolves during training. 
\paragraph{Compression Ratio} We study here whether the NTK evolves to compress diffeomorphisms. Following Eq.\ref{eq:R_f}, we define the NTK compression ratio 
\begin{equation}
    R_{NTK} = \frac{\langle \|\Theta(x, x) - \Theta(\tau x, x)\|^2\rangle_{x, \tau}}{\langle \|\Theta(x, x) - \Theta(x + \eta, x)\|^2\rangle_{x, \eta}},
\end{equation}
where again we impose $\|\tau x - x\| = \|\eta\|$.
\paragraph{Empirical Results} We measure the compression ratio for the neural tangent kernel computed after training for a ResNet18 and benchmark datasets. Results are shown in Figure \ref{fig:ntk_compression}; similarly to what we observe for the network function itself -- e.g. Figure \ref{fig:ntk_compression}-right and Figure \ref{fig:R_f}-panel3 -- we remark that also the NTK learns to compress directions corresponding to diffeomorphisms (full curves get below dashed ones).
% We measure compression of directions corresponding to diffeomorphisms for large enough values of $p$ (full curves under dashed ones).
\begin{figure}[hb]
    \centering
    \includegraphics[width=\linewidth]{figures/ntk_compression.pdf}
    \caption{\textbf{Compression ratio} at $\delta = 1$, $c=3$ for the NTK at initialization (dashed) and as a function of the train-set size $p$ (full) for a ResNet18 trained on MNIST (\vl{left}), FashionMNIST (\vl{center}) and CIFAR10 (\vl{right}). Compression magnitude gets larger with increasing $p$. The curves colors stand for different interpolation methods.}
    \label{fig:ntk_compression}
\end{figure}
\newpage

==> old sections/NetPredictions.tex <==
We provide here a connection between perturbations of the inputs and the prediction capabilities of trained networks. 

During training, a softmax function
\begin{equation}
    \hat{p}_i = \frac{e^{[f(x)]_i}}{\sum_j e^{[f(x)]_j}}
\end{equation}
is applied to the network output -- $[f(x)]_i$ indicates the i-th output entry of $f(x)$ -- and a cross-entropy loss function
\begin{equation}
    l = - \sum_c y_c^{\text{one-hot}} \log \hat{p}_c
\end{equation}
is minimized in order to have $\hat{p}$ match the one-hot encoding\footnote{If $C$ is the total number of classes, the labels $y$ take values in $\{1, \dots, C\}$ and a one-hot encoding of $y$ is a length-$C$ vector of 0's, with a 1 at entry $y$.} of $y$. 

In this context, the softmax output can be interpreted as the probability that the network gives to the input belonging to each of the classes. If we stick with this interpretation\footnote{There is some arbitrariness here: the fact that $\sum_i \hat{p}_i = 1$ doesn't imply that it makes sense to interpret the $\hat{p}_i$'s as probabilities -- or networks' uncertainty measures. Still, considering we are only interesting in the average relative changes of $\hat{p}_y$ when perturbing the inputs, we stay with the probability interpretation.}, we can compute how $\hat{p}_y$ (the probability that the network assigns to the true class) changes when the input is perturbed by Gaussian noise or smooth deformations, as a function of the temperature $T$, controlling the noise magnitude. In Figure \ref{fig:proba_resnet}, we report the average value of $\hat{p}_y$ over different input and noise samples, for a ResNet18. At $T\to 0$, $\langle \hat{p}_y\rangle$ is not dissimilar to the network test error (cf. Table \ref{tab:table1} in the Appendix), as it should be for it to be a good prediction uncertainty measure. As $T$ increases, we notice that the network prediction capabilities degrade quite fast under the application of Gaussian noise (dashed lines) while this is not the case for smooth deformations (full lines). When a diffeomorphism is applied, the network is able to correctly predict the true label even at large noise magnitudes (e.g. at $T=10$, $\hat{p}_y \approx 0.5$, large considering we have 10 classes), the better the smaller the cut-off $c$. Qualitatively, these results are in line with the measurements of the compression ratio in Section \ref{sec::compression-p}.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/proba_resnet.pdf}
    \caption{\textbf{Correct class prediction probability $\hat{p}_y$.} Average value of $\hat{p}_y$ for different input images and Gaussian noise (dashed) or diffeomorphism (full) samples as a function of $T$. Colors correspond to different interpolation methods. For diffeomorphisms, we report three high-frequency cut-off values $c$ (color intensity).
    At small $T$, the net's prediction is only slightly affected by the perturbations. As $T$ increases, the net's prediction capabilities degrade faster for Gaussian noise than for diffeomorphisms. For smooth deformations, the lower the cut-off, the more robust the network is to perturbations.}
    \label{fig:proba_resnet}
\end{figure}
